Frequency Dependent Vertex Functions of the (t,t')-Hubbard Model at Weak Coupling

We present a functional renormalization group calculation for the two-dimensional (t,t')-Hubbard model at Van Hove filling. Using a channel decomposition we describe the momentum and frequency dependence of the vertex function in the normal phase. Compared to previous studies that neglect frequency dependences we find higher pseudo-critical scales and a smaller region of d-wave superconductivity. A large contribution to the effective interaction is given by a forward scattering process with finite frequency exchange. We test different frequency parameterizations and in a second calculation include the frequency dependence of the imaginary self-energy. We also generalize the channel decomposition to frequency-dependent fermion-boson vertex functions.

==> sector-discretisation.tex <==
% draw sector discretisation segments in 1/8 of Brillouin zone
%
% need \usepackage{tikz}

\begin{tikzpicture}[x=1cm,y=1cm] 
   \draw[fill=gray!8] (0,0) node[anchor=north]{$\left(0,0\right)$} -- (5,0) node[anchor=north]{$\left(0,\pi\right)$} -- (5,5) node[anchor=west]{$\left(\pi,\pi\right)$} -- cycle;
   \draw (0, 0) -- (0,5) -- (5,5);
   \draw (5,0) -- (intersection of 5,0 -- 0,5 and 0,0 -- 5,5);
   \foreach \r in {1.18,2.36,3.54} {
      \draw (\r,0) arc (0:45:\r); 
      \draw (5,5-\r) arc (270:225:\r);
   }
   \draw (22.5:1.18)  -- (22.5:3.54) ;
   \draw[xshift=5cm, yshift=5cm] (247.5:1.18)  --  (247.5:3.54) ;
   \foreach \r in {0,1.18,2.36} {
     \draw (\r,0) circle(0.8mm);
     \draw[xshift=5cm, yshift=5cm] (0, -\r) circle(0.8mm);
   }
   \foreach \r in {1.18,2.36,3.54} {
     \draw (22.5:\r) circle(0.8mm);
     \draw[xshift=5cm, yshift=5cm] (247.5:\r) circle(0.8mm);
   }
\end{tikzpicture}


% \begin{tikzpicture}[
%   decoration={markings,mark=at position 0.5 with {\fill (2pt,0)--(-2pt,2.31pt)--(-2pt,-2.31pt)--cycle;}},
%    ]
%    \draw[postaction={decorate}] (0,0.2) -- (1,0.2);
%    \draw[postaction={decorate}] (1,-0.2) -- (0,-0.2);
% \end{tikzpicture}

